Location-Aware Visual Question Generation with Lightweight Models

This work introduces a novel task, location-aware visual question generation (LocaVQG), which aims to generate engaging questions from data relevant to a particular geographical location. Specifically, we represent such location-aware information with surrounding images and a GPS coordinate. To tackle this task, we present a dataset generation pipeline that leverages GPT-4 to produce diverse and sophisticated questions. Then, we aim to learn a lightweight model that can address the LocaVQG task and fit on an edge device, such as a mobile phone. To this end, we propose a method which can reliably generate engaging questions from location-aware information. Our proposed method outperforms baselines regarding human evaluation (e.g., engagement, grounding, coherence) and automatic evaluation metrics (e.g., BERTScore, ROUGE-2). Moreover, we conduct extensive ablation studies to justify our proposed techniques for both generating the dataset and solving the task.

==> fig_text/hists_q_quality.tex <==
%\begin{table*}[t]
%\centering
%    \begin{tabular}[c c]
%    \begin{minipage}{0.35\paperwidth}
%    \centering
%    \includegraphics[width=\linewidth]{images/Figure_4_3_revised.pdf}   
%    \caption{\textbf{Average Question Length (Token)}}
 %   \label{fig:hist_q_token_len}    
%    \end{minipage}
    
%    \hfill
    
%    \begin{minipage}{0.35\paperwidth}
%    \centering
%    \includegraphics[width=\linewidth]{images/Figure_4_4_revised.pdf}   
%    \caption{\textbf{Average Question Length (Sentence)}}
%    \label{fig:hist_q_sen_len}    
%    \end{minipage}
    
%    \hfill    
    
%    \begin{minipage}{0.3\paperwidth}
%    \centering
%    \scalebox{0.5}{!}{
%    \begin{tabular}{l c c}
%    \hline
%    Criterias & MVQG & Our Dataset \\
%    \hline
%    Vocab Size $\uparrow$ & 608 & \textbf{3046}  \\ 
%    Avg Sent. Length $\uparrow$ & 12.341 & \textbf{17.168} \\ 
%    Yngve score $\uparrow$ & 2.271 & \textbf{3.761} \\
%    \% Abstract Terms $\uparrow$ & 0.127 & \textbf{0.167} \\
%    Avg Term Depth $\downarrow$ & 7.906 & \textbf{7.259} \\
%    \hline
%    \end{tabular}
%    }
%    \caption{\textbf{Question Quality Comparison with MVQG}. $\uparrow$ indicates the score is better %higher, while $\downarrow$ is the other way around.}
%%    \label{comparison}
%    \end{minipage}
%    
%    \end{tabular}
%\end{table*}

\begin{figure*}[t]
  \begin{minipage}[t]{0.34\linewidth}
    \centering
	% \begin{subfig}{0.6\linewidth}
	% 	\includegraphics[width=\linewidth]{images/q_len_token.png}
	% 	\label{fig:hist_q_token_len}
	% \end{subfig}
	% \begin{subfig}{0.3\linewidth}
	% 	\includegraphics[width=\linewidth]{images/q_len_sen.png}
	% 	\label{fig:hist_q_sen_len}
 %        \end{subfig}  
    \includegraphics[width=\linewidth]{images/q_len_token.png}
    \caption{\textbf{Average Question Length}} %  (Token)}}
    \label{fig:hist_q_token_len}   
  \end{minipage}
  % \hfill
  \begin{minipage}[t]{0.17\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/q_len_sen.png}
    % \caption{\textbf{Average Question Length (Sentence)}}
    \label{fig:hist_q_sen_len}   
  \end{minipage}
  \begin{minipage}[t]{0.40\linewidth}
    \centering
    \scalebox{0.8}{\begin{tabular}{l c c}
    \hline
    Criterias & MVQG & Our Dataset \\
    \hline
    Vocab Size $\uparrow$ & 608 & \textbf{3046}  \\ 
    Avg Sent. Length $\uparrow$ & 12.341 & \textbf{17.168} \\ 
    Yngve score $\uparrow$ & 2.271 & \textbf{3.761} \\
    \% Abstract Terms $\uparrow$ & 0.127 & \textbf{0.167} \\
    Avg Term Depth $\downarrow$ & 7.906 & \textbf{7.259} \\
    \hline
    \end{tabular}}
    \caption{\textbf{Question Quality Comparison with MVQG}. $\uparrow$ indicates the score is better higher, while $\downarrow$ is the other way around.}
    \label{comparison}
  \end{minipage}
\end{figure*}

==> fig_text/q_len_stat.tex <==
\begin{figure*}[t]
  \begin{minipage}[t]{0.45\linewidth}
    \centering
    \includegraphics[width=0.64\linewidth]{images/q_len_token.png}
    \hfill
    \includegraphics[width=0.32\linewidth]{images/q_len_sen.png}
    \caption{\textbf{Length of Questions.}
    }
    \label{fig:hist_q_len}   
  \end{minipage}\hfill
  \begin{minipage}[t]{0.45\linewidth}
    \centering
    \scalebox{0.8}{\begin{tabular}{l l}
        \hline
        Statistic \\
        \hline
        \# of Image Sequences & 3759\\
        - \# of Image Sequences from Pittsburgh & 919\\
        - \# of Image Sequences from Orlando & 611\\
        - \# of Image Sequences from New York & 2217\\
        \# of Questions After Filtering & 35551 \\
        Average Sentence Length &  16.6 \\
        Average Question Length &  17.1 \\
        \hline
    \end{tabular}}
    \caption{\textbf{Dataset Statistic.}}
    \label{table:stats}
  \end{minipage}
\end{figure*}

==> problem.tex <==
\section{Problem Definition}

\textbf{Location-Aware Multi-VQG} We defined our problem, Location-Aware Multi-VQG, as a problem in which we used 
\subsection{Location Information}
